Learn to Segment Retinal Lesions and Beyond

Towards automated retinal screening, this paper makes an endeavor to simultaneously achieve pixel-level retinal lesion segmentation and image-level disease classification. Such a multi-task approach is crucial for accurate and clinically interpretable disease diagnosis. Prior art is insufficient due to three challenges, i.e., lesions lacking objective boundaries, clinical importance of lesions irrelevant to their size, and the lack of one-to-one correspondence between lesion and disease classes. This paper attacks the three challenges in the context of diabetic retinopathy (DR) grading. We propose Lesion-Net, a new variant of fully convolutional networks, with its expansive path re-designed to tackle the first challenge. A dual Dice loss that leverages both semantic segmentation and image classification losses is introduced to resolve the second challenge. Lastly, we build a multi-task network that employs Lesion-Net as a side-attention branch for both DR grading and result interpretation. A set of 12K fundus images is manually segmented by 45 ophthalmologists for 8 DR-related lesions, resulting in 290K manual segments in total. Extensive experiments on this large-scale dataset show that our proposed approach surpasses the prior art for multiple tasks including lesion segmentation, lesion classification and DR grading

==> Learn to Segment Retinal Lesions and Beyond/ablation.tex <==
%------------------------------------------------------------
%\subsubsection{Experiment 5. Ablation Study}  \label{sssec:exp-abla}
%------------------------------------------------------------




%\textbf{Attention}. 
%We compare the proposed SiAN with more alternatives. First, we compare different positions of adding attention weights. One is weighing the input image by element-wise multiplication. The other is weighing the intermediate feature maps. We will refer them as pre-fusion and post-fusion. Second, we compare different methods of getting attention weights, as mentioned in Eq. \ref{eq:att-w1} and Eq. \ref{eq:att-w2}.



%Results in \ref{tab:att} shows that SiAN obtains the best performance within all alternatives. The method that adopt Eq. \ref{eq:att-w2} to get attention weights and weighing the feature maps has slightly exceeded Inception-v3 (0.774) which shows that using Eq. \ref{eq:att-w1} to get attention weights can be helpful. However, it is not the best way as we mentioned in 3.2 that not only the regions with lesions, but also the leisons without lesion may helpful for DR grading.


An ablation study concerning the attention strategies is provided in Table \ref{tab:att}. Fusion at the feature map level is better than fusion at the input image. The better performance of learned weights supports our statement that a region deemed to be negative with respect to the lesions does not necessarily mean it is useless for DR grading.


\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Ablation study on attention strategies in SiAN}. L-Net-16s is used.}
\label{tab:att}
\scalebox{0.6}{
\begin{tabular}{@{}ll r r @{}}
\toprule
\multirow{2}{*}{\textbf{Fusion position}} && \multicolumn{2}{c}{\textbf{Attention weights}} \\
\cmidrule{3-4}
 && CW-MaxPool (Eq. \ref{eq:att-w1}) & Conv (Eq. \ref{eq:att-w2}) \\
\cmidrule{1-1} \cmidrule{3-4}
Input image            && 0.768 & 0.768 \\
Feature maps           && 0.781 & \textbf{0.803} \\

\bottomrule
\end{tabular}}
\end{table}





==> Learn to Segment Retinal Lesions and Beyond/approach.tex <==

Given a color fundus image, we aim to perform lesion segmentation, classification and subsequently DR grading in a unified framework. We use $\mathcal{X}$ to denote a specific $s \times s$ image, which contains an array of $s^2$ pixels $\{x_1,\ldots,x_i,\ldots,x_{s^2}\}$. Let $\mathcal{L}=\{l_1,\ldots,\l_m\}$ be $m$ lesions in consideration. Regions of distinct lesions, \eg, HaEx and iHE, often overlap partially, meaning a pixel can be assigned with multiple labels. So the goal of lesion segmentation is to automatically assign to each pixel $x_i$  a $m$-dimensional probabilistic vector, $\mathbf{p}_i=\{p_{i,1}, \ldots, p_{i,m}\}$, where $p_{i,j} \in [0,1]$ indicates the probability of the pixel belonging to the $j$-th lesion. 
%A binary label is obtained by thresholding at $0.5$. 
%
Lesion classification is to predict lesions at the image level. Given the probabilistic segmentation map $\{\mathbf{p}_1, \ldots, \mathbf{p}_{s^2}\}$, the probability of the presence of a specific lesion $l_j$, denoted as $P_j$, is naturally obtained by global max pooling on the map, \ie,
\begin{equation} \label{eq:Pj}
P_j := \max\{p_{1,j}, \ldots, p_{s^2,j} \},~~~j=1,\ldots,m.
\end{equation}
For both lesion segmentation and classification, hard labels are obtained by thresholding at $0.5$.
%
As for DR grading, the goal is to exclusively assign one of the following labels, \ie, \{DR0, DR1, DR2, DR3, DR4\}, to the given image. 

Next, we  depict the proposed lesion segmentation network, followed by the multi-task network. % its use for DR grading. 


\subsection{Lesion-Net for Retinal Lesion Segmentation} \label{ssec:lesion-seg-net}

%Our variant of FCN, as Fig. \ref{fig:l-net} shows, has a shorter expansive path, making the overall shape resemble the letter \textit{L}, which is also the initial of the word \emph{lesion}. We thus term the new segmentation network Lesion-Net. 
%Our proposed Lesion-Net is shown in Fig. \ref{fig:l-net}.

\begin{figure*} [tb!]
\centering
\includegraphics[width=1.9\columnwidth]{figures/grading}
\caption{
\textbf{Proposed multi-task network for (1) lesion segmentation, (2) lesion classification and (3) DR grading}. Given a color fundus image, % of size $3 \times 896 \times 896$, 
Lesion-Net-16s (the lower branch) generates probabilistic segmentation maps for eight lesions. Lesion classification is accomplished by global max pooling on the maps. For lesion-enhanced DR grading, a side-attention branch is used to fuse the segmentation maps with an array of 2,048 feature maps from  Inception-v3 in the upper branch. Compared with directly weighing the feature maps with the segmentation maps, the trainable side-attention is more effective.
%The trainable side-attention is more effective than directlying 
%Compared with directly weighing the feature maps with the segmentation maps, the side-attention branch 
%The upper branch is an Inception-v3 to generate an array of 2,048 feature maps, while the lower branch is an Lesion-Net to generate lesion maps. 
%Fusion at the feature map level leverages both semantic and spatial information of lesions. 
%In the contracting path (left side) of the network are the convolutional blocks of Inception-v3. Our novel design is the expansive path (right side). While adopting the U-Net's copy-and-merge strategy to re-use feature maps from the contractive path, for upsampling we substitute a $1 \times 1$ convolution for U-Net's deconvolution to adjust the number of feature maps and subsequently a parameter-free bilinear interpolation to increase the size of the feature maps. The length of our expansive path can be easily adjusted to handle lesion segmentation with imprecise boundaries.
}
\label{fig:l-net}
\vspace{-6mm}
\end{figure*}


\begin{figure} [tb!]
\centering
\includegraphics[width=1\columnwidth]{figures/l-net}
\caption{
\textbf{Variants of Lesion-Net}. The variable-length expansive path enables learning from lesion annotations with imprecise boundaries.}
\label{fig:l-net-settings}
\vspace{-7mm}
\end{figure}

\textbf{Network architecture}. 
For the contracting path of Lesion-Net, we use convolutional blocks of Inception-v3 \cite{inception-v3} for its outstanding feature extraction ability. Note that other state-of-the-art CNNs \cite{resnet,densenet,icml19-efficientnet} can, in principle, be used. 


Our task-specific design lies in the expansive path, where we leverage the effectiveness of U-Net \cite{unet} for re-using information from the contracting path and the flexibility of the original FCN \cite{fcn} in cutting off the expansive path for preventing over-precise segmentation. 

In concrete, in order to  re-use feature maps from the contracting path, we adopt U-Net's copy-and-merge strategy instead of adding operations in the FCN, see Fig. \ref{fig:l-net}. For upsampling, we replace U-Net's deconvolution by a $1 \times 1$ convolution to adjust the number of feature maps and subsequently a parameter-free bilinear interpolation to enlarge the feature maps. Such a tactic not only reduces the number of parameters. By applying an element-wise sigmoid activation, the output of the $1 \times 1$ convolution is naturally transformed to $m$ probabilistic maps with respect to the $m$ lesions. 


The fact that retinal lesions lack accurate boundaries makes it unnecessary to seek for very precise segmentation. While the symmetry between the contracting and expansive paths in U-Net is useful in its original context of cell segmentation, we argue that such a constraint is unnecessary for the current task. In fact, extra parameters introduced by the symmetry into the expansive path increases the difficulty of training the network. Therefore, we let the length of Lesion-Net's expansive path adjustable. If the expansive path is cut at an early stage with feature maps of size $28 \times 28$, the maps need to be upsampled by a factor of $32$ to produce the final segmentation maps. Following the convention of \cite{fcn}, we term this variant Lesion-Net-32s. By contrast, Lesion-Net-2s exploits all the intermediate feature maps. The models that fall in between are Lesion-Net-16s, Lesion-Net-8s and Lesion-Net-4s. 
Fig. \ref{fig:l-net-settings} shows Lesion-Net with distinct expansive paths. 


\textbf{Loss function}. 
Training Lesion-Net is nontrivial due to the following two issues.
First, while the area of a specific lesion varies, the importance of the lesion does not depend on its size. This property cannot be well reflected in a pixel-wise loss, to which a smaller blob contributes less. 
%As exemplified in Table \ref{tab:dual-loss}, 
Misclassifying a small blob does not lead to a significant increase in the segmentation loss, and thus difficult to be corrected during training. Such a small misclassification, even though ignorable from the viewpoint of semantic segmentation, can be crucial for proper diagnosis of related diseases.
Second, the data is extremely imbalanced, making commonly used loss functions such as cross entropy ineffective. Our study on a set of 12k expert-labeled fundus images shows that pixels of lesions account for less than 1\%. By contrast, for PASCAL VOC2012 \cite{ijcv15-voc}, a popular benchmark set for natural image segmentation, the proportion of pixels corresponding to objects is about 25\%. We find in preliminary experiments that with the cross-entropy loss, the lesion segmentation model easily got trapped in a local optimum, predicting all pixels as negative, albeit a very low training loss.

%\input{table-dual-loss}

To jointly address the two issues, we introduce a new \emph{dual loss} that combines a semantic segmentation loss $loss_{seg}$ and an image classification loss $loss_{clf}$, \ie,
%
\begin{equation}\label{eq:dual-loss}
loss_{dual} = \lambda \cdot loss_{seg} + (1 - \lambda) \cdot loss_{clf},
\end{equation}
where $\lambda \in [0,1]$ is a hyper parameter to strike a balance between the two sub-losses. 
%In principle, 
We instantiate both $loss_{seg}$ and $loss_{clf}$
% can be instantiated with any existing segmentation loss, and any classification loss for $loss_{clf}$. 
using the Dice loss, previously used for segmenting prostate MRI~\cite{vnet} and optic disc / cup~\cite{tmi18-mnet}. Our ablation study in Section \ref{sssec:exp-lesion-seg} shows that Dice loss is more effective than Weighed Cross Entropy~\cite{gdice} and Focal Loss~\cite{iccv17-focal}. The weight $\lambda$ is empirically set to $0.8$ based on a held-out validation set, a common practice for selecting hyper parameters. 

Note that the dual Dice loss is conceptually different from the multi-scale Dice \cite{tmi18-mnet}, which combines pixel-level Dice losses computed from images of varied scales and thus remains insensitive to small-sized errors. The motivation of 
our dual loss also differs from the combined cross-entropy loss described in \cite{zhang2018unified}, where the image classification loss is used as a regularization term to reduce overfitting. 

%To address the first issue, we adopt a pixel-level Dice loss, previously used for prostate MRI segmentation \cite{vnet}. 
Given a mini-batch of $n$ images, we compute the Dice version of $loss_{seg}$ as
\begin{equation} \label{eq:dice-pix}
loss_{seg} = 1 - \dfrac{2 \cdot \sum_{i=1}^{n \cdot s^2}{\sum_{j=1}^{m}{p_{i,j} \cdot t_{i,j}}}}{\sum_{i=1}^{n \cdot s^2}{\sum_{j=1}^{m}{p_{i,j}^2}} + \sum_{i=1}^{n \cdot s^2}{\sum_{j=1}^{m}{t_{i,j}^2}}},
\end{equation}
where $t_{i,j} \in \{0,1\}$ is ground truth of the $i$-th pixel with respect to the $j$-th lesion. In the extreme case where all pixels are predicted as negative, the dice loss is close to $1$.

We compute the Dice version of $loss_{clf}$ as 
\begin{equation} \label{eq:dice-img}
loss_{clf} = 1 - \dfrac{2 \cdot \sum_{i=1}^{n}{\sum_{j=1}^{m}{P_{i,j} \cdot T_{i,j}}}}{\sum_{i=1}^{n}{\sum_{j=1}^{m}{P_{i,j}^2}} + \sum_{i=1}^{n}{\sum_{j=1}^{m}{T_{i,j}^2}}},
\end{equation}
where $T_{i,j} \in \{0,1\}$ is the ground-truth label indicating whether the $j$-th lesion is present in the $i$-th image in the given batch. Recall that both $P_{i,j}$ and $T_{i,j}$ are obtained by global max pooling on the pixel-level labels, so $P_{i,j}$, $T_{i,j}$ and accordingly $loss_{clf}$ are all invariant to the lesion size.




%While image classification losses are used for weakly supervised semantic segmentation~\cite{wildcat,Wang_2018_CVPR}, where only image-level annotations are given, we are unaware of any previous work on exploiting both semantic segmentation and image classification losses for supervised semantic segmentation.

%
%
%Apparently, using $loss_{im}$ alone is problematic as the spatial information is completely lost. We propose a dual loss defined as 
%The two challenges are jointly addressed by training Lesion-Net to minimize a dual loss, \ie,  
%
%To discriminate an Lesion-Net trained with $loss_{ms}$, its counterpart trained using $loss_{px}$ will be postfixed with \emph{px}, \eg, Lesion-Net-4spx, Lesion-Net-8spx or Lesion-Net-16spx. 

%We show an example of the diffence between $loss_{px}$ and $loss_{im}$ for better understanding.



\subsection{Multi-task Network for Lesion-enhanced DR Grading} \label{ssec:grading-net}

To predict DR grades, we choose Inception-v3 \cite{inception-v3} as our baseline model. This model has established the state-of-the-art for predicting referable DR \cite{referable}, age-related eye diseases \cite{amd-deep} and other retinal abnormalities~\cite{miccai19-multidis}. In fact, for all models evaluated in this work, we use Inception-v3 as their backbones for fair comparison. To produce a probabilistic score per DR grade, we modify Inception-v3 by adding after the global average pooling (GAP) layer a fully connected layer of size $2,048 \times 5$, followed by a softmax layer.  Different from previous works that use a typical resolution of $299\times 299$ \cite{referable}, we use a much larger resolution of $896 \times 896$, making our Inception-v3 a much stronger baseline.


%We term this solution Concat-Net.
%We term the resultant network Concat-Net.

%We are goning to provide two different architectures trying to increase DR grading performance by using lesion predictions. One adopts lesion classification results into DR grading and the other adopts lesion segmentation results into DR grading.

%In the former architecture, an input image will first get a $m$-dimensional probabilistic vector $P = [P_1, P_2, \ldots ,P_m]$ indicating the probability of the presence of $m$ lesions. Then the input go through an Inception-V3 network to get a 2,048-dimensional feature vector $V$. Then $P$ and $V$ are concatenated together to get a $m+2048$-dimensional feature vector. At last, a fully connected layer is used to get the final DR grading score. We refer this architecture Concat-Net.

%Concat-Net ignores spatial information of the segmented lesions. 

%In order to exploit both semantic and spatial information of the segmented lesions, 

For lesion-enhanced DR grading, we propose a multi-task network, with its overall architecture shown in Fig. \ref{fig:l-net}. The multi-task network consists of two branches. At the top is its main branch, with Inception-v3 as the backbone, that performs DR grading. The side-attention branch, with Lesion-Net as its backbone, is responsible for injecting semantic and spatial information contained in the $m$ lesion segmentation maps into the main branch. In particular, the injection is performed at the last feature maps, denoted as $\{f_1,\ldots,f_{k}\}$, in the main branch, with $k=2,048$. To that end, the side-attention branch shall generate the same number of weight maps, denoted as $\{w_1,\ldots,w_{k}\}$. Multiplying the feature maps by the weight maps side by side generates new weighted feature maps as 
\begin{equation}
\{f_1 \otimes w_1, f_2 \otimes w_2, \ldots, f_{k} \otimes w_{k}\},
\end{equation}
where $\otimes$ indicates element-wise multiplication. The new feature maps then go through a GAP layer, followed by a classification block. 
It is worth point out that the weight information is essentially from the side-attention branch rather than generated by the main branch itself. Hence, the multi-task network is conceptually different from self-attention networks~\cite{nips17-atten,abn,cvpr19-danet}. 


%generating attention weights from the $m$ lesion segmentation maps. A fusion layer is used to inject the weights into the last $28\times 28$ feature maps, denoted as $\{f_1,\ldots,f_{2048}\}$, in the main branch. 

%works as a feature extractor to  generate an array of $2,048$ feature maps . The lower branch, with Lesion-Net as its backbone, is  A side-attention branch is used to inject the lesion maps into the feature maps. 

%as side information

To convert the lesion segmentation maps $\{s_1, \ldots, s_m\}$ into the weight maps, an intuitive strategy is to let the main branch pay attention to regions with maximal lesion response. This is achieved by channel-wise max pooling (CW-MaxPool) over the segmentation maps\footnote{The segmentation maps here are already down-sampled to the same size as the feature maps in the main branch.}, \ie
\begin{equation} \label{eq:att-w1}
w_i := \mbox{CW-MaxPool}(\{s_1, \ldots, s_m\}),~~~i=1,\ldots,k.
\end{equation} 
However, a region deemed to be negative with respect to the lesions does not necessarily mean it is useless for DR grading. So we further consider a learning based strategy, using a lightweight convolutional block consisting of two $3\times 3$ convolutional layers, \ie
\begin{equation} \label{eq:att-w2}
\{w_1,\ldots,w_k\} := \mbox{Conv}(\{s_1, \ldots, s_m\}).
\end{equation}
We train the multi-task network with the cross-entropy loss, commonly used for multi-class image classification.

 %attention is to let the main branch focuses o


%Concerning the choice of weights, a relatively straightforward strategy is to use probabilistic scores 

%%
 %, we propose \emph{Side-attention} Net, which performs fusion at the feature-map level and thus with the spatial information well preserved. As shown in Fig. \ref{fig:l-net}, \emph{Side-attention} Net  It is worth pointing out that directly weighing either the input image or the feature maps by the lesion maps is problematic. 

 %Therefore, we employ two $3\times 3$ convolutions to transform the lesion maps into $2,048$ weight maps $\{w_1,\ldots,w_{2048}\}$. Multiplying the feature maps by the weight maps side by side generates new weighted feature maps as 
%\begin{equation}
%\{f_1 \otimes w_1, f_2 \otimes w_2, \ldots, f_{2048} \otimes w_{2048}\},
%\end{equation}
%where $\otimes$ indicates element-wise multiplication. The new feature maps go through a GAP layer, followed by a classification block. All the three models, \ie, Inception-v3, Concat-Net and \emph{Side-attention} Net , are trained with the cross-entropy loss, commonly used for multi-class classification.







==> Learn to Segment Retinal Lesions and Beyond/exp-dr.tex <==

\textbf{Baselines}. We again compare with Inception-v3 and ABN, both re-trained for DR grading.
% Furthermore, we compare with ABN which is a self-attention model.
One might also consider a more straightforward method that enriches the output of the GAP layer by concatenating the $m$-dimensional lesion vector $(P_1, \ldots, P_m)$. Accordingly, the size of the fully connected layer is adjusted to $(2,048+m) \times 5$. Note that similar ideas have been exploited in the context of image captioning for obtaining semantically enhanced image features~\cite{tmm2019-cococn}. We term this baseline Lesion-Concat.


%\textbf{Performance metric}. We report the quadratic weighted \emph{kappa}, which measures inter-annotator agreement and used by the Kaggle DR Detection task \cite{kaggle}.  

\textbf{Results}. We use Lesion-Net-16s in the multi-task network for its best overall performance in the previous experiments. As Table \ref{tab:grading} shows, using a better lesion segmentation model results in more accurate DR grading,
%more accurate DR gradingbetter DR grading performance
%SiAN (Lesion-Net-16s)  outperforms all the baselines. 
%The better performance of SiAN against Concat-Net justifies the importance of fusion at the feature map level. Moreover, 
%Better lesion results lead to better DR grading. 
%We replace Lesion-Net-16s by other lesion segmentation models alternatives including U-Net, FCN-8s and DeepLabv3+, respectively, finding 
with the multi-task network (Lesion-Net-16s) as the top performer.
The better performance of learned weights (Eq. \ref{eq:att-w2}) compared to CW-MaxPool (Eq. \ref{eq:att-w1}) supports our statement that a region deemed to be negative with respect to the lesions does not necessarily mean it is useless for DR grading
%While ABN-grading has a relatively close performance, it is single-task. More importantly, its attention maps lack correspondence to manually marked lesion regions.

%More importantly, we observe that its attention maps lack correspondence to manually marked lesion regions, see Fig. \ref{fig:seg-map}.

%Further more, Table \ref{tab:grading} shows the importance of high resolution input images for reason that small lesions such as MA and iHE can not be seen in low resolution images.

\input{table-dr}

%\begin{figure} [tb!]
%\centering
%\includegraphics[width=\columnwidth]{./figures/compare_attention}
%\caption{
%\textbf{Visualizing DR grading results}. Compared to ABN's attention maps, lesion maps by our multi-task network better match ground truth. } 
%\label{fig:seg-map}
%\end{figure}


%\input{ablation}

We summarize the performance in Table \ref{tab:perf-overview}. When compared to the best baseline per task, the improvement seems to be not significant. However, for the best overall performance, one has to simultaneously deploy three distinct baselines (FCN-8s, DeepLabv3+ and ABN-grading) with 3.2GB GPU memory at run time, while our multi-task network performs better in all three tasks with half GPU memory (1.5GB).

\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Overall performance of different models}.}
\label{tab:perf-overview}
\vspace{-3mm}

\scalebox{0.78}{
\begin{tabular}{@{}ll l l r@{}}
\toprule
\textbf{Model}   &  \textbf{Lesion segmentation}  & \textbf{Lesion Classification} & \textbf{DR grading} \\
\hline
FCN-8s                           & 0.586 & 0.778 & - \\
DeepLabv3+                        & 0.553 & 0.794 & - \\
%\hline
%ABN lesion                        & n/a   & 0.726 & n/a \\
ABN-grading                       & -   & -   & 0.797 \\
%\hline
%SiAN (FCN-8s)         & 0.586 & 0.778 & 0.787 \\
%\hline
%SiAN (DeepLabv3+)    & 0.553 & 0.794 & 0.787 \\
\emph{Our model}  & \textbf{0.591} & \textbf{0.801} & \textbf{0.803} \\
\bottomrule
\end{tabular}}
\vspace{-6mm}
\end{table}






==> Learn to Segment Retinal Lesions and Beyond/exp-inc.tex <==

~\\* 
\textbf{Performance metric}. %To measure the inconsistency between the predicted lesions and DR grade per test image, 
Based on Table \ref{tab:DRLevel}, we compile a set of simplified rules in Table \ref{tab:inc-rules}.  We report the inconsistency rate (\emph{IncRate}), namely the percentage of images with inconsistent DR grading and lesion predictions.

\input{table-inc-rule}

\textbf{Results}. Table \ref{tab:inc_rate} shows the IncRate matrix between different lesion prediction models and DR grading models. Comparing the columns corresponding to L-Net-16spx and L-Net-16s, the latter consistently has lower IncRate. So, adding the image-level Dice loss is beneficial for generating more consistent lesion and DR grade predictions. Both Concat-Net and SiAN have lower IncRate than Inception-v3, suggesting that lesion-enhanced DR grading is also helpful for making more consistent predictions. Given the best IncRate of around 20\%, there is much room for future improvement. 



%\begin{table} [tb!]
%\renewcommand{\arraystretch}{1}
%\centering
%\caption{\textbf{The IncRate matrix between different lesion classification models and DR grading models}. \xr{to be updated}}
%\label{tab:inc_rate}
%\scalebox{0.7}{
%\begin{tabular}{@{}ll r r r r@{}}
%\toprule
%& \multicolumn{5}{| c |}{ } \\
%\multirow{2}{*}{\textbf{DR grading}} && \multicolumn{4}{c}{\textbf{Lesion classification}} \\
%\cmidrule{3-5}
% && Inception-v3 & ABN  &  FCN-32s  & L-Net-16s \\
%\multirow{5}{*}{\begin{sideways}{\small \textbf{DR grading model}}\end{sideways}}
%\cmidrule{1-1} \cmidrule{3-5}
%Inception-v3                && 0.225  & 0.195          & 0.264          & 0.235 \\
%ABN                         && 0.214  & 0.193          & 0.xxx          & 0.xxx \\
%Lesion-Concat (L-Net-16s)   && 0.218  & 0.193          & 0.242          & 0.210 \\
SiAN (FCN-32s)              && 0.208  & 0.183          & 0.225          & 0.195 \\
SiAN (L-Net-16s)            && 0.220  & 0.201          & 0.241          & 0.212 \\


\bottomrule
\end{tabular}}
\end{table}



%Figure \ref{fig:consistancy} shows some examples of DR grading and how the lesion segmentation results help FusionNet to get the consistent and correct DR grades.
%\input{inc-figure}

==> Learn to Segment Retinal Lesions and Beyond/exp-lesion-clf.tex <==
%~\\* 
\textbf{Baselines}. We re-use the baselines from Experiment 1, with lesion classification obtained by global max pooling on segmentations. We also compare with two segmentation-free models, \ie, Inception-v3~\cite{inception-v3} and ABN~\cite{abn}, both trained using image-level lesion annotations and Dice.

%with the Dice and binary cross entropy losses, respectively.  We refer to them as Inception-v3 (Dice), Inception-v3 (BCE), ABN(Dice) and ABN(BCE).

%\textbf{Performance metric}. Image-wise F1 is used.


\textbf{Comparing Lesion-Net with distinct settings}. As Table \ref{tab:lesion-seg} shows, for lesion classification Lesion-Net with a shorter expansive path, \eg~Lesion-Net-16s and Lesion-Net-32s, is preferred. From Table \ref{tab:lesion-seg} we see that Lesion-Net trained with the dual loss is the best, suggesting small misclassified blobs are reduced. 

%\input{table-lesion-clf}


\textbf{Comparing with the baselines}. Inception-v3 and ABN are less effective than the majority of the segmentation based models. The results suggest the importance of lesions' spatial information even for making image-level predictions. Different from its behavior for lesion segmentation, DeepLabv3+ becomes runner-up for lesion classification. For vHE, this model outperforms the others with a large margin. Note that DeepLabv3+ is specifically designed to capture multi-scale information by its parallel dialated convolutions. This design appears to be good at capturing the major pattern of vHE which often occupies more than half of an image. Overall Lesion-Net-16s is the best.



==> Learn to Segment Retinal Lesions and Beyond/exp-lesion-seg.tex <==
%~\\*
\input{table-lesion-seg}


\textbf{Baselines}. Our criteria for choosing baselines are two-fold: state-of-the-art in related tasks and open-source, allowing us to run them with the same preciseness as intended by their developers. Four prior arts, \ie, FCN \cite{fcn}, U-Net~\cite{unet}, DeepLabv3+~\cite{deeplabv3p}, 
%CE-Net~\cite{gu2019net}, 
and DANet~\cite{cvpr19-danet}, are compared. For all networks, we use Inception-v3 as the backbone of their contracting paths.
%
%We compare with four prior arts, \ie, FCN \cite{fcn}, U-Net~\cite{unet}, DeepLabv3+~\cite{deeplabv3p},  CE-Net~\cite{gu2019net}, and DANet~\cite{cvpr19-danet}. To let the comparison focus on the expansive paths, for all networks we use Inception-v3 as the backbone of their contracting paths.
%, \ie,~Inception-v3. 
In addition, as the majority of the existing works utilize a patch-based sliding window approach to detect retinal lesions, we include patch-based FCN-32s. To train the patch-based model, we uniformly divide each image into $4\times4$ patches, each sized to 224$\times$224. Given a test image, the model is run with a window size of $224\times224$ and a stride of $112$. Scores from overlapped areas are averaged. 
All the baselines are trained with the Dice loss. 

%Note that, given the same backbone (Inception-v3), Lesion-Net-32s and FCN-32s are the same in architecture. In the following experiments, the two models are distinguished by the loss funcetions. FCN-32s is trained with Dice loss while Lesion-Net-32s is trained with Dual loss if not specially clarified.

%\textbf{Performance metric}. Pixel-wise F1 score is reported.
% precision and recall are computed per lesion. In order to measure the performance using one metric, we report F1, the harmonic average of precision and recall. 



\textbf{Comparing Lesion-Net with distinct settings}. 
%From Lesion-Net-32s to Lesion-Net-2s, the expansive path of Lesion-Net goes deeper and the parameters increase. 
As Table \ref{tab:lesion-seg} shows, the overall performance of Lesion-Net increases first, from 0.573 (Lesion-Net-32s) to 0.591 (Lesion-Net-16s), and decreases later, from 0.592 (Lesion-Net-4s ) to 0.581 (Lesion-Net-2s). The peak is obtained by Lesion-Net-8s, with an F1 of 0.603. The result confirms our hypothesis that when the network parameters keep increasing, the additional layers can have a negative effect on the performance. 


%Concerning the losses, recall that the F1 metric is computed as the pixel level. 


\textbf{Comparing loss functions}. 
%We compare with Dice~\cite{vnet}, Focal loss~\cite{iccv17-focal}, and weighted cross-entropy (WCE) \cite{gdice}. 
As the parameter $\alpha$ in Focal loss~\cite{iccv17-focal} is dataset-dependent, we set it to $0.8$ according to our validation set, with the parameter $\gamma$ set to $2$ as suggested in the original paper. Dice and the proposed dual loss outperform Focal and WCE\cite{gdice} with a large margin, see Table \ref{tab:lesion-seg}. Correcting small-sized errors cannot be well reflected by the pixel-wise F1 score. This explains the relatively small difference between Dice and the dual loss for lesion segmentation.

%we set $\alpha=0.8$ according to our validation set and follow the author's suggestion to set $\gamma=2$. Results are shown in Tab. \ref{tab:loss}. Dice loss and the Dice based Dual loss achieve much more better performances in lesion segmentation and classification whose data is extremely unbalanced. Moreover, in order to solve the data unbalance, the parameter $\alpha$ in focal loss has to adjusted according to the data distribution while Dice loss and Dual loss can adaptively solve the problem. Dual loss achieves better classification performances because is takes classification loss into account.

%\input{table-loss}

%Correcting small-sized errors is not well reflected by the pixel-wise F1 metric. This explains the marginal difference between Lesion-Nets trained using distinct losses, see for instance Lesion-Net-4s and Lesion-Net-4spx (0.592 versus 0.590). Recall that an Lesion-Net postfixed with \emph{px} means training using $loss_{px}$.



\textbf{Comparing with the baselines}. Lesion-Net outperforms the baselines. 
%The lower performance of U-Net suggests the difficulty of training a lesion segmentation model from scratch. 
Patch-based FCN-32s is less effective than its full-resolution counterpart. As noted in Section \ref{sec:related}, properly recognizing MA requires a holistic view, which is absent for the patch-based model. This explains its lowest performance (F1 of 0.209) on this lesion. Patch-based FCN-32s also has difficulty in segmenting large lesions such as vHE and pHE.
%
Compared to DeepLabv3+, Lesion-Net shows similar performance on MA, iHE, HaEx and CWS while noticeably better for vHE, pHE, NV and FiP. Comparing the two groups of lesions, the latter lack clear boundaries. As shown in Fig. \ref{fig:sup_example}, irregular segmentation boundaries produced by DeepLabv3+ implies its attempt to produce precise boundaries, which are however unnecessary for retinal lesions. The results confirm our hypothesis that DeepLabv3+ is over-designed for this task. In the meantime, the viability of the proposed Lesion-Net for retinal lesion segmentation is justified.
%Moreover, We notice that CE-Net show competitive performance on small lesions such as MA, iHE and HaEx, while failed to detect other lesions at all. All the pixels are predicted as background for the rest 5 lesions.


\begin{figure*} [tbh!]
\centering
\includegraphics[width=1.8\columnwidth]{figures/sup_examples_v2}
\vspace{-3mm}
\caption{
\textbf{Some qualitative results of lesion segmentation and classification}. Red font indicates false alarms. The proposed Lesion-Net-16s produces more smooth segmentation boundaries and less false alarms. Best viewed digitally.}
\label{fig:sup_example}
\vspace{-6mm}
\end{figure*}


==> Learn to Segment Retinal Lesions and Beyond/experiment.tex <==


%============================================================
\subsection{Experimental Setup} \label{ssec:setup}
%============================================================


\input{lesions}

%\subsubsection{Implementations}

\textbf{Implementations}. An input image is sized to $896 \times 896$, as small lesions can not be seen well in lower resolution. We use SGD with a weight decay factor of $0.0001$ and a momentum of $0.95$. The initial learning rate is $0.001$. Validation occurs every 1K batches. If the validation performance does not improve in 4 consecutive validations, the learning rate will be divided by $10$. Early stop occurs once the performance does not improve in 10 consecutive validations. 
For training Lesion-Net, 
we start with $loss_{seg}$. Once the learning rate is reduced, $loss_{seg}$ is replaced by $loss_{dual}$. For DR grading, a pre-trained Lesion-Net is used for the multi-task network. We tried to train both branches, but found no improvement in DR grading yet an absolute decrease of 0.01 in the segmentation performance. So we did not go further in that direction. For the varied models assessed in this paper, we use Inception-v3 pre-trained on ImageNet~\cite{cvpr09-imagenet} as their backbones. Random rotation, crop, flip and random changes in brightness, saturation and contrast are used for data augmentation. Training was performed using PyTorch on two NVIDA Tesla P40 GPUs. 

\textbf{Evaluation criteria}. For lesion segmentation, we report pixel-wise F1 score, the harmonic mean of precision and recall. For lesion classification, we report image-wise F1. As lesions predicted at the pixel level are propagated to the image level via global max pooling, the two criteria complements each other, providing a more comprehensive assessment of a specific segmentation model. For DR grading, We report the quadratic weighted \emph{kappa}, which measures inter-annotator agreement and used by the Kaggle DR Detection task~\cite{kaggle}. 
%Once trained, running the multi-task network takes about 1.5GB GPU memory.

%Our criteria for choosing baseline methods are two-fold:  state-of-the-art in related tasks and open-source, allowing us to run them with the same preciseness as intended by their developers.


%============================================================
%\subsection{Experiments} \label{ssec:exp}
%============================================================

%------------------------------------------------------------
\subsection{Experiment 1. Lesion Segmentation} \label{sssec:exp-lesion-seg}
%------------------------------------------------------------

\input{exp-lesion-seg}
\input{more-analysis}

%------------------------------------------------------------
\subsection{Experiment 2. Lesion Classification} \label{sssec:exp-lesion-det}
%------------------------------------------------------------

\input{exp-lesion-clf}

%------------------------------------------------------------
\subsection{Experiment 3. Lesions for DR Grading} \label{sssec:exp-dr}
%------------------------------------------------------------

\input{exp-dr}





%------------------------------------------------------------
%%\subsubsection{Experiment 4. Inconsistency between Lesion Prediction and DR Grading}  \label{sssec:exp-inc}
%------------------------------------------------------------

%\input{exp-inc}







==> Learn to Segment Retinal Lesions and Beyond/intro.tex <==

%The goal of this paper is to simultaneously resolve two computer vision tasks, \ie~\emph{semantic segmentation} and \emph{image classification}, in the context of color fundus images. 
%Color fundus photography is the most widely used measure for retinal screening and early detection of vision-threatening diseases such as diabetic retinopathy, age-related macular degeneration and glaucoma. 
Given the increasing demand of retinal screening and the clear shortage of experienced ophthalmologists, fundus image based retinal disease diagnosis is crucial for the well-being of many~\cite{referable,miccai19-multidis,miccai19-amd}.
%
Previous studies on fundus image segmentation concentrate on anatomical structures in retina including optic disc / cup and vessels \cite{tmi18-mnet,tmi19-cenet,cvprw19-m2u-net}. By contrast, this paper aims for \emph{retinal lesions}, which are symptoms of ocular fundus diseases manifested in color fundus images. By answering the question of what lesions are in a fundus image and where in the image they are located, lesion segmentation has a potential to enable clinical interpretability of disease classes predicted at the image level. Attacking lesion segmentation and retinal disease classification in a unified framework is thus valuable.

Note that for natural images as in PASCAL-VOC alike tasks \cite{wildcat,Ge_2018_CVPR,Zhou_2018_CVPR}, the semantic segmentation task and the image classification task typically share the same class vocabulary. Consequently, developing a multi-task approach seems to be relatively straightforward, \eg, by converting classes predicted at the pixel-level to the image-level by max or mean pooling.
%, as illustrated in Fig. \ref{fig:sketch}~(a). 
For fundus images, however, lesion labels and disease classes are distinct and lack one-to-one correspondence. See for instance lesions used in the clinical practice guidelines for diabetic retinopathy\footnote{Diabetic retinopathy is a complication of diabetes mellitus caused by damage to blood vessels of the light-sensitive tissue at the retina \cite{dc17-dr}.} (DR) grading in Table \ref{tab:DRLevel}.
%The connection between lesions and diseases resembles that between attributes and categories in natural images. 
This means lesion segmentation cannot be directly converted to image-level DR grades. 
%Besides class discrepancy, a side effect of having both lesion and disease predictions is inevitably inconsistency between the two, an issue overlooked in the literature~\cite{fleming2010role,niemeijer2007automated}. 
Hence, a unified framework that  effectively segments lesions and exploits the segmentation for accurate disease classification is in demand.



%\begin{figure} [tb!]
%\centering
%\includegraphics[width=0.9\columnwidth]{figures/sketch_map}
%\caption{\textbf{Fundus versus natural images in a multi-task setting}. Unlike natural images where segmentation results can be easily converted to image labels, the fact that retinal lesions and diseases lack one-to-one correspondence makes it nontrivial to exploit lesion segmentation for disease prediction.}\label{fig:sketch}
%\end{figure}


\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{A summary of the American Academy of Ophthalmology (AAO) preferred practice pattern guidelines for diabetic retinopathy grading}. As venous beading and IrMA are very difficult to be recognized even for ophthalmologists and occur rarely, we exclude them from this study. The eight lesions stuided in this work are indicated by \cmark.}
\label{tab:DRLevel}
\scalebox{0.9}{
\begin{tabular}{@{} l |l | l @{}}
\toprule
\textbf{Grade} & \multicolumn{2}{c}{\textbf{Lesion evidence for DR grading}} \\
\hline
               & \emph{Sufficient} & \emph{Indirect} \\
\hline
%DR0 && No abnormalities & - \\
DR1 & $\bullet$ Microaneurysm (MA), exclusively \cmark & -- \\
\hline
DR2 & $\bullet$ Intraretinal hemorrhage (iHE) \cmark & $\bullet$ Hard exudate (HaEx) \cmark \\
\hline
DR3 & \specialcell{Any of the following:\\ 
                     $\bullet$ Over 20 iHEs in each of 4 quadrants \\
                     $\bullet$ Venous beading in 2+ quadrants \\
                     $\bullet$ IrMA in 1+ quadrants} & \specialcell{$\bullet$ Cotton-wool spot \\ (CWS) \cmark} \\ 
\hline
DR4 & \specialcell{Any of the following:\\
                     $\bullet$ Neovascularization (NV) \cmark \\
                     $\bullet$ Vitreous hemorrhage (vHE) \cmark \\
                     $\bullet$ Preretinal hemorrhage (pHE) \cmark} & \specialcell{$\bullet$ Fibrous proliferation\\ (FiP) \cmark} \\

\bottomrule
\end{tabular}}
\vspace{-6mm}
\end{table}


%\xr{to re-write. Besides the social impact, a multi-task approach to semantic segmentation and image classification is scientifically interesting yet technically challenging.} this paper emphasizes \emph{retinal lesion segmentation}, an upstream task in fundus image analysis.







%This paper targets at \emph{retinal lesion segmentation}, a challenging task in medical image analysis. 
%Moreover, multiple lesion classes can co-present in the same image, with their regions (partially) overlapped. In order to answer the question of what lesions are in a fundus image and where in the image they are located, pixel-level multi-label classification is required. As such, retinal lesion segmentation seems to be a specific case of semantic image segmentation.


Given a fundus image, instances of a specific lesion class occupy a specific region or multiple regions with diverse visual appearance, see Fig. \ref{fig:example}. 
With the advent of fully convolutional networks (FCN) \cite{fcn}, exciting progress has been made in semantic segmentation, especially for natural scenes~\cite{dialated,segnet,deeplabv3p,cvpr19-danet,iccv19-ccnet}. However, directly applying the state-of-the-art for retinal lesion segmentation is problematic. %questionable. % due to the following three challenges. %unique properties of the task. 
%First, 
Unlike objects in natural images, retinal lesions lack clear boundaries against the background. It is practically impossible for ophthalmologists to segment lesions at the same preciseness, meaning an FCN has to learn from annotations with imprecise boundaries. In the meanwhile, for diagnosis, it is mostly the presence and locality of specific lesions that are involved, see Table \ref{tab:DRLevel}. 
%See for instance the clinical practice guidelines for diabetic retinopathy (DR) grading in Table \ref{tab:DRLevel}. 
Extremely precise segmentation is not only difficult to achieve but also unnecessary from a clinical view. We thus hypothesize that cutting-edge FCNs, \eg, DeepLabv3+~\cite{deeplabv3p}, are over-designed for lesion segmentation.


\begin{figure} [tb!]
\centering
\includegraphics[width=\columnwidth]{figures/examples-reduced}
\caption{
\textbf{Visual examples of 8 DR-related retinal lesions studied in this paper}. For a clear view, we show only one lesion per image.}
%\textbf{Retinal lesions with manual / automated segmentations}. For better viewing, we show only one lesion per image. For lesions with relatively clear boundaries, \ie, microaneurysm (MA), intraretinal hemorrhage (iHE), hard exudate (HaEx), and cotton-wool spot (CWS), the proposed Lesion-Net is on par with DeepLabv3+. As for lesions lacking clear boundaries, \ie, vitreous hemorrhage (vHE), preretinal hemorrhage (pHE), neovascularization (NV) and fibrous proliferation (FiP), Lesion-Net achieves better segmentation. Best viewed on screen.}
\label{fig:example}
\vspace{-6mm}
\end{figure}

Moreover, while the importance of an object in a natural image is largely reflected by its size~\cite{cvpr12-berg-import}, the importance of a lesion in a fundus image does not count on the amount of pixels it possesses. Diabetic retinopathy, depending on what lesions are presented, is categorized into five levels, from DR0 (\ie, no DR) to DR4~(\ie, proliferative DR). 
The presence of a preretinal hemorrhage, even though in a relatively small size, means DR4. Such a property cannot be well addressed by current segmentation losses including cross entropy \cite{fcn,unet,cvpr18-seg-every}, focal loss~\cite{iccv17-focal,Yu_2018_CVPR}, and Dice \cite{vnet,tmi18-mnet}.
%, commonly used to train FCN based semantic segmentation models. 

%Third, while semantic segmentation is a standalone task, retinal lesion segmentation has to go one step further to prove its value for disease diagnosis. A desirable FCN shall not only aim for lesion segmentation, but also generate output that can be flexibly integrated into another (deep) model for disease diagnosis. As shown in Fig. \ref{fig:sketch}, In contrast to traditional PASCAL-VOC alike tasks \cite{wildcat}, for fundus images pixel-level and image-level labels are distinct. The connection between lesions and diseases resembles that between attributes and categories in natural images. It implies lesion segmentation cannot be directly converted to image-level DR grades, and vice versa. Moreover, a side effect of having both lesion and disease predictions is inevitably inconsistency between the two. The inconsistency issue is overlooked \cite{fleming2010role,niemeijer2007automated}. 


To conquer the aforementioned challenges, this paper makes the first endeavor to simultaneously solve retinal lesion segmentation and disease classification in an end-to-end framework. We choose DR, a leading cause of blindness~\cite{dc17-dr}, as our target disease. Our main novelties are 


%\begin{itemize}

$\bullet$ We study eight lesions including microaneurysm (MA), intraretinal hemorrhage (iHE), hard exudate (HaEx), cotton-wool spot (CWS), vitreous hemorrhage (vHE), preretinal hemorrhage (pHE), neovascularization (NV), and fibrous proliferation (FiP) that support the full range of DR grades. This is a new state-of-the-art in terms of quantity, complexity and clinical usability.

$\bullet$ We propose Lesion-Net for retinal lesion segmentation. While inheriting FCN's classical contracting-and-expansive structure, Lesion-Net has a re-designed expansive path with its length adjustable and its upsampling operation lightweight trainable. We adopt a \emph{dual loss} that combines both semantic segmentation and image classification losses. These two designs enable Lesion-Net to effectively learn from lesion annotations with imprecise boundaries and to substantially reduce false alarms of small-size lesions. 

%The design enable Lesion-Net to effectively learn from lesion annotations with imprecise boundaries.


% Naturally inspired by state-of-the-art semantic segmentation, Lesion-Net's main novelty lies in its architecture and loss for fulfilling the requirements in the new domain. Different from U-Net and DeepLabv3+, Lesion-Net has an adjustable expansive path with lightweight trainable upsampling for learning to segment lesions with imprecise boundaries. We design a dual loss that combines pixel- and image-level losses to neatly handle severe data imbalance.

$\bullet$ We propose a multi-task network that effectively harnesses lesion segmentation maps, as side information, for improving DR grading. Such an attention mechanism conceptually differs from prevalent self-attention mechanisms~\cite{nips17-atten,abn,cvpr19-danet}. Once trained, the multi-task network performs three tasks, \ie, lesion segmentation, lesion classification and DR grading, all in one forward pass. 

%utilizing lesion segmentation for improving DR grading. \emph{Side-attention} Net effectively converts lesion labels predicted at pixel-level to image-level DR grades. 


$\bullet$ We conduct extensive experiments on 12K color fundus images collected from Kaggle \cite{kaggle} and local hospitals. With 290K expert-labeled pixel-level lesion segments, the dataset is the largest of its kind. The experiments confirm the superiority of both Lesion-Net and the multi-task network against the prior art including FCN~\cite{fcn}, U-Net~\cite{unet}, DANet~\cite{cvpr19-danet}, and DeepLabv3+~\cite{deeplabv3p} for lesion segmentation and classification, Inception-v3~\cite{inception-v3} and ABN~\cite{abn} for DR grading. 
To promote related research, we have released the Kaggle part of our test data, containing 1,593 images and 34,268 expert-labeled lesion segments\footnote{\url{https://github.com/WeiQijie/retinal-lesions}}, substantially larger than the present-day dataset that has only 81 images with manual segmentation for four lesions~\cite{mia20-idrid}.

%To promote related research, the Kaggle part of our test data, containing 1,593 images and 34,268 expert-labeled lesion segments, will be released. 

%the new FCN outperforms the original FCN \cite{fcn}, U-Net \cite{unet} and DeepLabv3+ \cite{deeplabv3p} for lesion segmentation. The fusion network improves over Inception-v3 \cite{inception-v3} for DR grading, and reduces inconsistency between lesion and DR results. 

%\item Last, we fuse the most lesions into DR grading and achieve better DR grading performance and we make the first attempt to evaluate the consistency between lesions and DR grading.
%\end{itemize}





==> Learn to Segment Retinal Lesions and Beyond/lesions.tex <==

%\subsubsection{Data}


%\textbf{Lesion selection}. 
According to the AAO guidelines \cite{aao2017}, there are seven lesions used as sufficient evidence for specific DR grades. Among them, venous beading and IrMA are very difficult to be recognized even for ophthalmologists and occur rarely. So they are excluded from this study. We include three other lesions, \ie,~HaEx, CWS, and FiP, indirectly related to DR grading. 
%The three lesions alone shall not be considered as a sign of DR. However, they become informative once cooccuring with lesions directly related to DR. For instance, HaEx is lipids as a consequence of hemorrhages, so images with HaEx and MA are likely to be graded as DR2. When an image is observed with many DR2-related evidences, the presence of a CWS shall lift the grade from DR2 to DR3. New vessels in the retinal may undergo fibrosis and form FiPs. Therefore, a FiP is often considered to be a sign of DR4 when it does not occur alone. 
We compile a final list of eight lesions, see Table \ref{tab:DRLevel}.


\textbf{Ground-truth construction}. Public datasets suited for our purpose does not exist. So we construct a large collection of 12,252 color fundus images with both pixel-level lesion annotations and image-level DR grades as follows. 
%
We collected initially 23K color fundus images of posterior pole, consisting of 12k images from our hospital partners and 11k images randomly sampled from the Kaggle DR Detection task \cite{kaggle}. While the images were from patients with diabetes, some of them show other eye diseases such as glaucoma, AMD and RVO. So DR0 does not necessarily mean a healthy eye. Such a characteristic makes the data close to the real scenario and thus challenging. 

For expert labeling, a panel of 45 experienced ophthalmologists was formed. We developed a web-based annotation system, where an annotator marks out  lesions in a given image using either ellipses or polygons and accordingly grade the image. Lesion annotation and DR grading from a single image are somewhat subjective. So for quality control, each image was assigned to at least three annotators. Images receiving consistent DR grades, \ie,~the majority vote for a specific grade, are preserved. Accordingly, per image we cleaned lesion annotations so they are complied to the diagnostic guidelines. Eventually, we obtain 12,252 images with 290K expert-labeled lesion segments. We split the dataset at random for training (70\%), validation (10\%) and test (20\%). 
%Basic statistics are visualized in Figure \ref{fig:dataset}. Furthermore, 
%Table \ref{tab:co-occ} shows co-occurrence between DR grades and lesions. 

%To make the annotations more reliable, we first exclude images that only receive 1 annotation. Furthermore, only images that receive consistent DR grading level in more than half of the annotations are reserved. The ground-truth of an image for DR grading is the most of all its DR grading level annotations. The ground-truth of an image for lesion segmentation is the union set of all its lesion annotations because we think that doctors get easier to miss some small lesions rather than misclassify backgrounds into lesions.


%\input{data-stat-fig}






==> Learn to Segment Retinal Lesions and Beyond/more-analysis.tex <==
%\subsubsection{More analysis on various pathologies}

%\begin{figure*} [h!]
%\scalebox{2.5}{\centering
%\includegraphics[width=0.85\columnwidth]{figures/sup_examples}}
%\caption{
%\textbf{Some qualitative results}. Ground truth is expert-labeled lesion segments. \emph{ABN grading} denotes the ABN model trained for the DR grading task, while \emph{ABN lesion} means the ABN model trained for the lesion classification task. Note the nearly uniform attention maps by ABN lesion (the 4th column), suggesting its attention mechanism has little influence for lesion classification. As for ABN grading, there is lack of correspondence between its attended regions and the real lesion areas. Also note the irregular segmentation boundaries produced by DeepLabv3+ (the 6th column), implying its attempt to produce precise boundaries, which are however unnecessary for retinal lesions. Overall the proposed L-Net-16s (the 9th column) produces more smooth segmentation boundaries and less false alarms. Best viewed on screen.}
%\label{fig:sup_example}
%\end{figure*}

\begin{figure} [tbh!]
\centering
\includegraphics[width=0.9\columnwidth]{figures/seg-perf}
\vspace{-3mm}
\caption{Illustrating Table \ref{tab:lesion-seg}, lesions sorted by their average size.}
\label{fig:seg-perf}
\vspace{-4mm}
\end{figure}


As shown in Fig. \ref{fig:seg-perf}, for small-sized lesions with relatively clear boundaries (MA, iHE, CWS and HaEx), we observe close performance among distinct models. Exceptions are L-Net-32s and FCN-32s, as they do 32$\times$ upsampling by parameter-free bilinear interpolation, and thus difficult to accurately locate small lesions. For large lesions yet with imprecise boundaries (NV, pHD and vHE), the simplicity of FCN and L-Net becomes advantageous. The L-Net series produce more smooth segmentation boundaries. The fact that the top performer for FiP is L-Net-32s is due to the relatively clear boundary of this large lesion.


==> Learn to Segment Retinal Lesions and Beyond/related-work.tex <==
%We firsh discuss FCN based semantic segmentation. We then review progress in fundus image segmentation, followed by a discussion about lesion-enhanced DR grading. At last, we review the methods to simultaneously predict DR grades and lesions.

\textbf{Models for semantic segmentation}. 
Since Long \etal \cite{fcn}, FCNs have been the \emph{de facto} standard technique for semantic segmentation. An FCN can be conceptually decomposed into a contracting path and an expansive path. The contracting path progressively extracts and downsamples feature maps from an input image. The expansive path, by transforming and upsampling, produces a full-resolution segmentation map of the same size as the input image. Towards more precise segmentation, novel designs are continuously proposed either in the contracting path, or in the expansive path or in both. For instance, dilated convolutions are introduced in \cite{dialated}, so the contracting path can produce feature maps with higher resolutions to preserve more detailed spatial information. In U-Net \cite{unet}, the contracting path and the expansive path are carefully designed to be symmetrical. Skip connections from the contracting path to the expansive path are added, again for the purpose of preserving spatial information to generate more accurate segmentation boundaries. In order to capture long-range contextual information in both spatial and channel dimensions, DANet \cite{cvpr19-danet} introduces a position attention module and  a channel attention module in the expansive path. The state-of-the-art DeepLabv3+ uses both dilated convolutions and spatial pyramid pooling in its contracting path \cite{deeplabv3p}.  Its expansive path uses multiple skip connections to exploit features from lower levels. As identifying the precise boundary of a retinal lesion is secondary to the practical use of lesion segmentation, a new FCN is required.

%\textbf{Losses for semantic segmentation}. While standard cross entropy remains popular~\cite{fcn,unet,cvpr18-seg-every}, new losses are being invented, mainly for addressing class imbalance. Exemplars are weighted cross entropy~\cite{gdice}, Focal Loss~\cite{iccv17-focal}, and Dice \cite{vnet}, all computed at the pixel-level. A multi-scale Dice is used in~\cite{tmi18-mnet}, where an image is resized to multiple scales and pixel-level Dice losses computed at each scale are combined. Meanwhile, image classification losses are used for weakly supervised semantic segmentation~\cite{Ge_2018_CVPR,wildcat,cvpr16-cam,Wang_2018_CVPR}, where only image-level annotations are given. The joint use of both semantic segmentation and image classification losses is metioned in \cite{zhang2018unified}. The classification loss in \cite{zhang2018unified} is used as a regularization term to reduce overfitting. 


\textbf{Retinal lesion segmentation}. While earlier works for retinal lesion segmentation use traditional image processing techniques~\cite{fleming2010role,niemeijer2007automated}, current works mostly take a patch-based deep learning approach \cite{tmi16-hemorrhage-detection,ma-he-exudates,high-risk-lesions,miccai18-lesion-detction}. In \cite{tmi16-hemorrhage-detection}, for instance, a customized CNN is used to segment iHE by patch classification. Similarly in \cite{high-risk-lesions}, a patch-trained CNN is applied in a sliding window manner, classifying every grid in a test image into five classes, \ie, normal, MA, iHE, HaEx and high-risk lesion.  By predicting whether a given patch contains a specific lesion, segmentation maps obtained by the above works tend to be sparse and imprecise. A more fundamental drawback is that the approach lacks a holistic view. Consider MA and iHE for instance. The two lesions are visually close as both are small lesions look like dark dots. However, MA occurs around vessels. Also, an image with no other lesion is more likely to have MA than iHE. For a model looking only at local areas, modeling these kinds of holistic clues is difficult. 

\textbf{Lesion-enhanced DR grading}. 
%While the above works consider lesion segmentation as a standalone task, 
Initial efforts have been made towards lesion-enhanced DR grading. A two-step method is developed in \cite{lesion-dr1}, where an input image is first converted to a weight map by using a CNN to classify all patches of the image as normal, MA or iHE. The image, multiplied by the weight map, is fed into a DR grading network. A lesion-guided attention mechanism is described in \cite{lesion-dr2} to weigh specific regions in the input image. Three lesions are considered: MA, iHE and HaEx. Neither of these works considers severe lesions such as pHE, vHE, and NV. %Furthermore, when both lesions and DR grades are predicted, inconsistency occurs. For instance, an image might be graded as DR0, \ie, no apparent retinopathy, but in the meantime with MA detected. Such an consistency is not evaluated in the literature. 
%In \cite{zoom-in-net,aaai19-pathlogoical}, activation maps in a DR detection network are exploited to localize potential lesions. As their goal is to visualize pathological evidence used by the network, what lesions and to what extent they can be segmented are not quantitatively evaluated. 

%\cite{zoom-in-net}

\textbf{Attention-enhanced image classification}. The state-of-the-art is Attention Branch Network (ABN) \cite{abn}, which extends a response-based visual explanation model~\cite{cvpr16-cam} by introducing an attention branch into a specific CNN. Consequently, ABN not only improves image classification but also produces an attention map to interpret the decision. Note that the attention is self-generated. Our attention mechanism exploits the output of the semantic segmentation network as side information, and thus conceptually differs from ABN.


==> Learn to Segment Retinal Lesions and Beyond/table-dr-guidelines.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{A summary of the American Academy of Ophthalmology (AAO) preferred practice pattern guidelines for diabetic retinopathy grading}. As venous beading and IrMA are very difficult to be recognized even for ophthalmologists and occur rarely, we exclude them from this study. The eight lesions stuided in this work are indicated by \cmark.}
\label{tab:DRLevel}
\scalebox{0.7}{
\begin{tabular}{@{} |l |l | l| @{}}
\hline
\textbf{Grade} & \multicolumn{2}{c|}{\textbf{Lesion evidence for DR grading}} \\
\hline
               & \emph{Sufficient} & \emph{Indirect} \\
\hline
%DR0 && No abnormalities & - \\
DR1 & $\bullet$ Microaneurysm (MA), exclusively \cmark & -- \\
\hline
DR2 & $\bullet$ Intraretinal hemorrhage (iHE) \cmark & $\bullet$ Hard exudate (HaEx) \cmark \\
\hline
DR3 & \specialcell{Any of the following:\\ 
                     $\bullet$ Over 20 iHEs in each of 4 quadrants
                     $\bullet$ Venous beading in 2+ quadrants 
                     $\bullet$ IrMA in 1+ quadrants} & \specialcell{$\bullet$ Cotton-wool spot  (CWS) \cmark} \\ 
\hline
DR4 & \specialcell{Any of the following:\\
                     $\bullet$ Neovascularization (NV) \cmark 
                     $\bullet$ Vitreous hemorrhage (vHE) \cmark 
                     $\bullet$ Preretinal hemorrhage (pHE) \cmark} & \specialcell{$\bullet$ Fibrous proliferation (FiP) \cmark} \\

\hline
\end{tabular}}
\end{table}


==> Learn to Segment Retinal Lesions and Beyond/table-dr.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{DR grading results}. Numbers after Inception-v3 means the input resolution.}
\label{tab:grading}
\vspace{-3mm}
\scalebox{0.78}{
\begin{tabular}{@{}ll l l r@{}}
\toprule
\textbf{DR model} & \textbf{Attention weights}  &  \textbf{Lesion model}  && \textbf{Kappa}\\
\hline
Inception-v3 ($224\times 224$)  & --                                & --                && 0.660 \\
Inception-v3 ($488\times 448$)  & --                                & --                && 0.729 \\
Inception-v3                    & --                                & --                && 0.774 \\
Lesion-Concat                   & --                                & Inception-v3      && 0.780 \\
\emph{Multi-task network}       & Conv (Eq. \ref{eq:att-w2})        & U-Net             && 0.780 \\
\emph{Multi-task network}       & CW-MaxPool (Eq. \ref{eq:att-w1})  & Lesion-Net-16s    && 0.781 \\
\emph{Multi-task network}       & Conv (Eq. \ref{eq:att-w2})        & FCN-8s            && 0.787 \\
\emph{Multi-task network}       & Conv (Eq. \ref{eq:att-w2})        & DeepLabv3+        && 0.787 \\
Lesion-Concat                   & --                                & Lesion-Net-16s    && 0.788 \\
ABN-grading                     & --                                & --                && 0.797 \\
\emph{Multi-task network}       & Conv (Eq. \ref{eq:att-w2})        & Lesion-Net-16s    && \textbf{0.803}\\
\bottomrule
\end{tabular}}
\vspace{-6mm}
\end{table}


==> Learn to Segment Retinal Lesions and Beyond/table-dual-loss.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{Behavior of different losses}. With the image classification loss $loss_{clf}$ added, the proposed \emph{dual loss} $loss_{dual}$ is more sensitive to small-sized errors (bright spots in the second row).}%, than the pixel-level loss $loss_{px}$.}
\label{tab:dual-loss}
\scalebox{0.75}{
\begin{tabular}{@{} lll| lll|  l l l@{}}
\toprule
\multicolumn{2}{c}{\textbf{Ground-truth}} && \multicolumn{2}{c}{\textbf{Prediction}} && $loss_{seg}$ & $loss_{clf}$ & $loss_{dual}$\\
%\hline 
\multirow{2}{*}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multirow{2}{*}{\includegraphics[width=0.07\textwidth]{figures/8.png}} && \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/7.png}} && 0.0736 & 0.0  & 0.0589 \\ 
\cmidrule{4-9}
%\multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/8.png}} 
&&& \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/2.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/7.png}} && 0.0797 & 0.3325 & 0.1303 \\ 
 
\bottomrule
\end{tabular}}
\end{table}


==> Learn to Segment Retinal Lesions and Beyond/table-inc-rule.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{Rules to judge the inconsistency between predicted DR grades and lesions}. DR2 and DR3 share rules, since two DR3-related lesions, \ie., IrMA and venous beading, are excluded from this study and we do not count lesions.  CWS, HaEx and FiP are not included as they have no strict relation with the DR grades. }
\label{tab:inc-rules}
\scalebox{0.7}{
\begin{tabular}{@{} l |l @{}}
\toprule
\textbf{Grade} & \textbf{Rules} \\
\hline
DR0 & \specialcell{Any of the following predicted:
                             MA, iHE, vHE, pHE, NV} \\
\hline
DR1 & \specialcell{ No MA or any of the following predicted:
                             iHE, vHE, pHE, NV} \\
\hline
DR2, DR3 & \specialcell{Any of the following predicted:
                                  vHE, pHE, NV} \\
\hline
DR4 & \specialcell{None of the following predicted:
                                  vHE, pHE, NV} \\
\bottomrule
\end{tabular}}
\end{table}

==> Learn to Segment Retinal Lesions and Beyond/table-lesion-clf.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Lesion classification by different models}.}
\label{tab:lesion-clf}
\scalebox{0.8}{
\begin{tabular}{@{}ll r r r r r r r r r@{}}
\toprule
% \cmidrule{4-6} \cmidrule{8-10}
\textbf{Model} && \textbf{Mean} & MA    & iHE   & HaEx  & CWS   & vHE   & pHE   & NV    & FiP \\
\cmidrule{1-1} \cmidrule{3-11}
%\emph{Baselines} \\
patch FCN-32s       && 0.704          & 0.886          & 0.849          & 0.828          & 0.720          & 0.634          & 0.544          & 0.637          & 0.535 \\ 
FCN-32s             && 0.769          & 0.900          & 0.858          & 0.856          & 0.771          & 0.722          & 0.683          & 0.694          & 0.669 \\
FCN-16s             && 0.787          & 0.890          & 0.849          & 0.847          & 0.743          & 0.758          & 0.726          & 0.696          & 0.783 \\
FCN-8s              && 0.778          & 0.891          & 0.858          & 0.854          & 0.749          & 0.766          & 0.711          & 0.671          & 0.725 \\
U-Net               && 0.757          & 0.888          & 0.855          & 0.843          & 0.755          & 0.639          & 0.689          & 0.653          & 0.737 \\
DeepLabv3+          && 0.794          & 0.899          & 0.863          & 0.866          & 0.764          & \textbf{0.800} & 0.693          & 0.677          & 0.792 \\ 
DANet               && 0.775          & 0.900          & 0.853          & 0.852          & 0.772          & 0.713          & 0.682          & 0.715          & 0.712 \\ [3pt]

Inception-v3   && 0.716          & 0.895          & 0.893          & 0.865          & 0.766          & 0.500          & 0.540          & 0.594          & 0.678 \\ 
%ABN (BCE)           && 0.717          & \textbf{0.911} & 0.894          & 0.836          & 0.723          & 0.475          & 0.581          & 0.654          & 0.661 \\
%Inception-v3 (BCE)  && 0.719          & 0.900          & 0.897          & 0.858          & 0.759          & 0.475          & 0.556          & 0.623          & 0.682 \\
ABN-lesion && 0.726          & 0.900          & \textbf{0.900} & \textbf{0.871} & 0.761          & 0.519          & 0.552          & 0.627          & 0.678 \\ [3pt]

%\emph{Lesion-Net with Dice loss} \\
%Lesion-Net-8s            && 0.759          & 0.899          & 0.856          & 0.849          & 0.769          & 0.690          & 0.617          & 0.660          & 0.730 \\
%Lesion-Net-4s            && 0.765          & 0.900          & 0.862          & 0.849          & 0.763          & 0.674          & 0.645          & 0.655          & 0.771 \\
%Lesion-Net-2s            && 0.767          & 0.898          & 0.865          & 0.853          & 0.764          & 0.699          & 0.649          & 0.663          & 0.747 \\
%Lesion-Net-16s           && 0.769          & 0.899          & 0.860          & 0.851          & 0.754          & 0.709          & 0.661          & 0.694          & 0.724 \\

%\emph{Lesion-Net with Dual loss} \\
%Lesion-Net-32s  && 0.792          & 0.899          & 0.881          & 0.857          & 0.778          & 0.720          & \textbf{0.773} & 0.669          & 0.762 \\
Lesion-Net          && \textbf{0.801} & 0.902          & 0.882          & 0.866          & 0.792          & 0.733          & 0.726          & 0.701          & \textbf{0.807} \\
%Lesion-Net-8s            && 0.780          & 0.900          & 0.881          & 0.861          & 0.771          & 0.687          & 0.693          & 0.711          & 0.733 \\
%Lesion-Net-4s            && 0.781          & 0.904          & 0.883          & 0.862          & 0.791          & 0.678          & 0.660          & \textbf{0.719} & 0.748 \\
%Lesion-Net-2s            && 0.787          & 0.900          & 0.893          & 0.868          & \textbf{0.793} & 0.706          & 0.706          & 0.667          & 0.764 \\


\bottomrule
\end{tabular}}
\end{table}


==> Learn to Segment Retinal Lesions and Beyond/table-lesion-seg.tex <==
\begin{table*} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Lesion segmentation and classification by different models}.}
\label{tab:lesion-seg}
\scalebox{0.75}{
\begin{tabular}{@{}ll r r r r r r r r r r r r r r r r r r r@{}}
\toprule
% \cmidrule{4-6} \cmidrule{8-10}
\multirow{1}{*}{\textbf{Model}} && \multicolumn{9}{c}{Lesion segmentation} && \multicolumn{9}{c}{Lesion classification} \\
\cmidrule{3-11} \cmidrule{13-21}
&& \textbf{Mean} & MA    & iHE   & HaEx  & CWS   & vHE   & pHE   & NV & FiP && \textbf{Mean} & MA    & iHE   & HaEx  & CWS   & vHE   & pHE   & NV & FiP\\
\cmidrule{1-1} \cmidrule{3-11} \cmidrule{13-21}
%\emph{Baselines} \\
patch FCN-32s       && 0.553          & 0.209          & 0.583          & 0.714          & 0.535          & 0.622          & 0.549          & 0.554          & 0.659 
                    && 0.704          & 0.886          & 0.849          & 0.828          & 0.720          & 0.634          & 0.544          & 0.637          & 0.535\\
FCN-32s             && 0.571          & 0.327          & 0.592          & 0.728          & 0.528          & 0.642          & 0.562          & 0.530          & 0.662  
                    && 0.769          & 0.900          & 0.858          & 0.856          & 0.771          & 0.722          & 0.683          & 0.694          & 0.669\\
FCN-16s             && 0.587          & 0.369          & 0.608          & 0.737          & 0.575          & 0.639          & 0.515          & 0.581          & 0.671 
                    && 0.787          & 0.890          & 0.849          & 0.847          & 0.743          & 0.758          & 0.726          & 0.696          & 0.783\\
FCN-8s              && 0.586          & 0.369          & 0.609          & 0.740          & 0.573          & 0.640          & 0.534          & \textbf{0.583} & 0.639  
                    && 0.778          & 0.891          & 0.858          & 0.854          & 0.749          & 0.766          & 0.711          & 0.671          & 0.725\\

U-Net               && 0.570          & 0.384          & 0.598          & 0.730          & 0.565          & 0.547          & 0.604          & 0.538          & 0.592  
                    && 0.757          & 0.888          & 0.855          & 0.843          & 0.755          & 0.639          & 0.689          & 0.653          & 0.737\\

DeepLabv3+          && 0.553          & 0.367          & 0.612          & 0.732          & 0.558          & 0.550          & 0.477          & 0.498          & 0.631  
                    && 0.794          & 0.899          & 0.863          & 0.866          & 0.764          & \textbf{0.800} & 0.693          & 0.677          & 0.792\\ 
%CE-Net              && 0.219          & \textbf{0.402} & 0.612          & 0.738          & 0.0            & 0.0            & 0.0            & 0.0            & 0.0  
%                    && 0.325          & 0.886          & 0.853          & 0.859          & 0.0            & 0.0            & 0.0            & 0.0            & 0.0\\
DANet               && 0.585          & 0.351          & 0.608          & 0.733          & 0.560          & 0.623          & 0.589          & 0.543          & 0.671 
                    && 0.775          & 0.900          & 0.853          & 0.852          & 0.772          & 0.713          & 0.682          & 0.715          & 0.712\\ [3pt]

Inception-v3        && --             & --             & --             & --             & --             & --             & --             & --             & --
                    && 0.716          & 0.895          & 0.893          & 0.865          & 0.766          & 0.500          & 0.540          & 0.594          & 0.678 \\ 
ABN-lesion          && --             & --             & --             & --             & --             & --             & --             & --             & --
                    && 0.726          & 0.900          & \textbf{0.900} & \textbf{0.871} & 0.761          & 0.519          & 0.552          & 0.627          & 0.678 \\ [3pt]
\hline
\emph{Lesion-Net (Dual Dice loss)} \\
Lesion-Net-32s      && 0.573          & 0.289          & 0.590          & 0.730          & 0.539          & 0.632          & 0.536          & 0.582   & \textbf{0.687}
                    && 0.792          & 0.899          & 0.881          & 0.857          & 0.778          & 0.720          & \textbf{0.773} & 0.669          & 0.762 \\
Lesion-Net-16s      && 0.591          & 0.377          & 0.612          & 0.740          & 0.565          & 0.645          & 0.590          & 0.571         & 0.623
                    && \textbf{0.801} & 0.902          & 0.882          & 0.866          & 0.792          & 0.733          & 0.726          & 0.701   & \textbf{0.807}\\
Lesion-Net-8s       && \textbf{0.603} & 0.377          & \textbf{0.617} & 0.740          & 0.575          & \textbf{0.648} & \textbf{0.616} & 0.580          & 0.667 
                    && 0.780          & 0.900          & 0.881          & 0.861          & 0.771          & 0.687          & 0.693          & 0.711          & 0.733 \\
Lesion-Net-4s       && 0.592          & 0.394          & 0.614          & 0.743          & \textbf{0.577} & 0.633          & 0.588          & 0.570          & 0.616
                    && 0.781          & \textbf{0.904} & 0.883          & 0.862          & 0.791          & 0.678          & 0.660          & \textbf{0.719} & 0.748 \\
Lesion-Net-2s       && 0.581          & 0.381          & 0.614          & \textbf{0.744} & 0.567          & 0.634          & 0.569          & 0.565          & 0.572
                    && 0.787          & 0.900          & 0.893          & 0.868          & \textbf{0.793} & 0.706          & 0.706          & 0.667          & 0.764 \\




%\emph{Lesion-Net with Dual loss} \\
%Lesion-Net-32s      && 0.573          & 0.289          & 0.590          & 0.730          & 0.539          & 0.632          & 0.536          & 0.582          & \textbf{0.687} \\
\hline
Lesion-Net-16s (WCE)     && 0.364            & 0.180          & 0.389          & 0.543         & 0.346            & 0.424         & 0.245        & 0.363          & 0.423  
                    && 0.534            & 0.864         & 0.822         & 0.780         & 0.574             & 0.324         & 0.274         & 0.354         & 0.282\\
Lesion-Net-16s (Focal)   && 0.458             & 0.165         & 0.479         & 0.682         & 0.409             & 0.471         & 0.488         & 0.423         & 0.548
                    && 0.745             & 0.880         & 0.869         & 0.837         & 0.723             & 0.650         & 0.693         & 0.627         & 0.683\\
Lesion-Net-16s (Dice)    && 0.594          & 0.362          & 0.609          & 0.734          & 0.570          & 0.637          & 0.587          & 0.573          & 0.683 
                    && 0.769          & 0.899          & 0.860          & 0.851          & 0.754          & 0.709          & 0.661          & 0.694          & 0.724 \\

%Lesion-Net-8s      && \textbf{0.603} & 0.377          & \textbf{0.617} & 0.740          & 0.575          & \textbf{0.648} & \textbf{0.616} & 0.580          & 0.667 \\
%Lesion-Net-4s            && 0.592          & 0.394          & 0.614          & 0.743          & 0.577          & 0.633          & 0.588          & 0.570          & 0.616 \\
%Lesion-Net-2s            && 0.581          & 0.381          & 0.614          & \textbf{0.744} & 0.569          & 0.634          & 0.569          & 0.565          & 0.572 \\
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table*}


==> Learn to Segment Retinal Lesions and Beyond/table-loss.tex <==


\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Performance of Lesion-Net-16s with different losses}. }
\label{tab:loss}
\scalebox{0.9}{
\begin{tabular}{@{}ll r r@{}}
\toprule
\textbf{Loss}      && \textbf{Lesion segmentation} &\textbf{Lesion classification}    \\
\cmidrule{1-1}  \cmidrule{2-4}
\emph{Lesion-Net-16s}: \\
Weighted cross-entropy  && 0.365  & 0.533 \\
Focal loss              && 0.504  & 0.635 \\
Dice                && \textbf{0.594}  & 0.769 \\
\emph{Dual loss (this paper)}               && 0.591  & \textbf{0.801} \\ [3pt]

\bottomrule
\end{tabular}}
\end{table}

==> ablation.tex <==
%------------------------------------------------------------
%\subsubsection{Experiment 5. Ablation Study}  \label{sssec:exp-abla}
%------------------------------------------------------------




%\textbf{Attention}. 
%We compare the proposed SiAN with more alternatives. First, we compare different positions of adding attention weights. One is weighing the input image by element-wise multiplication. The other is weighing the intermediate feature maps. We will refer them as pre-fusion and post-fusion. Second, we compare different methods of getting attention weights, as mentioned in Eq. \ref{eq:att-w1} and Eq. \ref{eq:att-w2}.



%Results in \ref{tab:att} shows that SiAN obtains the best performance within all alternatives. The method that adopt Eq. \ref{eq:att-w2} to get attention weights and weighing the feature maps has slightly exceeded Inception-v3 (0.774) which shows that using Eq. \ref{eq:att-w1} to get attention weights can be helpful. However, it is not the best way as we mentioned in 3.2 that not only the regions with lesions, but also the leisons without lesion may helpful for DR grading.


An ablation study concerning the attention strategies is provided in Table \ref{tab:att}. Fusion at the feature map level is better than fusion at the input image. The better performance of learned weights supports our statement that a region deemed to be negative with respect to the lesions does not necessarily mean it is useless for DR grading.


\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Ablation study on attention strategies in SiAN}. L-Net-16s is used.}
\label{tab:att}
\scalebox{0.6}{
\begin{tabular}{@{}ll r r @{}}
\toprule
\multirow{2}{*}{\textbf{Fusion position}} && \multicolumn{2}{c}{\textbf{Attention weights}} \\
\cmidrule{3-4}
 && CW-MaxPool (Eq. \ref{eq:att-w1}) & Conv (Eq. \ref{eq:att-w2}) \\
\cmidrule{1-1} \cmidrule{3-4}
Input image            && 0.768 & 0.768 \\
Feature maps           && 0.781 & \textbf{0.803} \\

\bottomrule
\end{tabular}}
\end{table}





==> exp-inc.tex <==

~\\* 
\textbf{Performance metric}. %To measure the inconsistency between the predicted lesions and DR grade per test image, 
Based on Table \ref{tab:DRLevel}, we compile a set of simplified rules in Table \ref{tab:inc-rules}.  We report the inconsistency rate (\emph{IncRate}), namely the percentage of images with inconsistent DR grading and lesion predictions.

\input{table-inc-rule}

\textbf{Results}. Table \ref{tab:inc_rate} shows the IncRate matrix between different lesion prediction models and DR grading models. Comparing the columns corresponding to L-Net-16spx and L-Net-16s, the latter consistently has lower IncRate. So, adding the image-level Dice loss is beneficial for generating more consistent lesion and DR grade predictions. Both Concat-Net and SiAN have lower IncRate than Inception-v3, suggesting that lesion-enhanced DR grading is also helpful for making more consistent predictions. Given the best IncRate of around 20\%, there is much room for future improvement. 



%\begin{table} [tb!]
%\renewcommand{\arraystretch}{1}
%\centering
%\caption{\textbf{The IncRate matrix between different lesion classification models and DR grading models}. \xr{to be updated}}
%\label{tab:inc_rate}
%\scalebox{0.7}{
%\begin{tabular}{@{}ll r r r r@{}}
%\toprule
%& \multicolumn{5}{| c |}{ } \\
%\multirow{2}{*}{\textbf{DR grading}} && \multicolumn{4}{c}{\textbf{Lesion classification}} \\
%\cmidrule{3-5}
% && Inception-v3 & ABN  &  FCN-32s  & L-Net-16s \\
%\multirow{5}{*}{\begin{sideways}{\small \textbf{DR grading model}}\end{sideways}}
%\cmidrule{1-1} \cmidrule{3-5}
%Inception-v3                && 0.225  & 0.195          & 0.264          & 0.235 \\
%ABN                         && 0.214  & 0.193          & 0.xxx          & 0.xxx \\
%Lesion-Concat (L-Net-16s)   && 0.218  & 0.193          & 0.242          & 0.210 \\
SiAN (FCN-32s)              && 0.208  & 0.183          & 0.225          & 0.195 \\
SiAN (L-Net-16s)            && 0.220  & 0.201          & 0.241          & 0.212 \\


\bottomrule
\end{tabular}}
\end{table}



%Figure \ref{fig:consistancy} shows some examples of DR grading and how the lesion segmentation results help FusionNet to get the consistent and correct DR grades.
%\input{inc-figure}

==> table-dr-guidelines.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{A summary of the American Academy of Ophthalmology (AAO) preferred practice pattern guidelines for diabetic retinopathy grading}. As venous beading and IrMA are very difficult to be recognized even for ophthalmologists and occur rarely, we exclude them from this study. The eight lesions stuided in this work are indicated by \cmark.}
\label{tab:DRLevel}
\scalebox{0.7}{
\begin{tabular}{@{} |l |l | l| @{}}
\hline
\textbf{Grade} & \multicolumn{2}{c|}{\textbf{Lesion evidence for DR grading}} \\
\hline
               & \emph{Sufficient} & \emph{Indirect} \\
\hline
%DR0 && No abnormalities & - \\
DR1 & $\bullet$ Microaneurysm (MA), exclusively \cmark & -- \\
\hline
DR2 & $\bullet$ Intraretinal hemorrhage (iHE) \cmark & $\bullet$ Hard exudate (HaEx) \cmark \\
\hline
DR3 & \specialcell{Any of the following:\\ 
                     $\bullet$ Over 20 iHEs in each of 4 quadrants
                     $\bullet$ Venous beading in 2+ quadrants 
                     $\bullet$ IrMA in 1+ quadrants} & \specialcell{$\bullet$ Cotton-wool spot  (CWS) \cmark} \\ 
\hline
DR4 & \specialcell{Any of the following:\\
                     $\bullet$ Neovascularization (NV) \cmark 
                     $\bullet$ Vitreous hemorrhage (vHE) \cmark 
                     $\bullet$ Preretinal hemorrhage (pHE) \cmark} & \specialcell{$\bullet$ Fibrous proliferation (FiP) \cmark} \\

\hline
\end{tabular}}
\end{table}


==> table-dual-loss.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{Behavior of different losses}. With the image classification loss $loss_{clf}$ added, the proposed \emph{dual loss} $loss_{dual}$ is more sensitive to small-sized errors (bright spots in the second row).}%, than the pixel-level loss $loss_{px}$.}
\label{tab:dual-loss}
\scalebox{0.75}{
\begin{tabular}{@{} lll| lll|  l l l@{}}
\toprule
\multicolumn{2}{c}{\textbf{Ground-truth}} && \multicolumn{2}{c}{\textbf{Prediction}} && $loss_{seg}$ & $loss_{clf}$ & $loss_{dual}$\\
%\hline 
\multirow{2}{*}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multirow{2}{*}{\includegraphics[width=0.07\textwidth]{figures/8.png}} && \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/7.png}} && 0.0736 & 0.0  & 0.0589 \\ 
\cmidrule{4-9}
%\multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/1.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/8.png}} 
&&& \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/2.png}} & \multicolumn{1}{m{1cm}}{\includegraphics[width=0.07\textwidth]{figures/7.png}} && 0.0797 & 0.3325 & 0.1303 \\ 
 
\bottomrule
\end{tabular}}
\end{table}


==> table-inc-rule.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1}
\centering
\caption{\textbf{Rules to judge the inconsistency between predicted DR grades and lesions}. DR2 and DR3 share rules, since two DR3-related lesions, \ie., IrMA and venous beading, are excluded from this study and we do not count lesions.  CWS, HaEx and FiP are not included as they have no strict relation with the DR grades. }
\label{tab:inc-rules}
\scalebox{0.7}{
\begin{tabular}{@{} l |l @{}}
\toprule
\textbf{Grade} & \textbf{Rules} \\
\hline
DR0 & \specialcell{Any of the following predicted:
                             MA, iHE, vHE, pHE, NV} \\
\hline
DR1 & \specialcell{ No MA or any of the following predicted:
                             iHE, vHE, pHE, NV} \\
\hline
DR2, DR3 & \specialcell{Any of the following predicted:
                                  vHE, pHE, NV} \\
\hline
DR4 & \specialcell{None of the following predicted:
                                  vHE, pHE, NV} \\
\bottomrule
\end{tabular}}
\end{table}

==> table-lesion-clf.tex <==
\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Lesion classification by different models}.}
\label{tab:lesion-clf}
\scalebox{0.8}{
\begin{tabular}{@{}ll r r r r r r r r r@{}}
\toprule
% \cmidrule{4-6} \cmidrule{8-10}
\textbf{Model} && \textbf{Mean} & MA    & iHE   & HaEx  & CWS   & vHE   & pHE   & NV    & FiP \\
\cmidrule{1-1} \cmidrule{3-11}
%\emph{Baselines} \\
patch FCN-32s       && 0.704          & 0.886          & 0.849          & 0.828          & 0.720          & 0.634          & 0.544          & 0.637          & 0.535 \\ 
FCN-32s             && 0.769          & 0.900          & 0.858          & 0.856          & 0.771          & 0.722          & 0.683          & 0.694          & 0.669 \\
FCN-16s             && 0.787          & 0.890          & 0.849          & 0.847          & 0.743          & 0.758          & 0.726          & 0.696          & 0.783 \\
FCN-8s              && 0.778          & 0.891          & 0.858          & 0.854          & 0.749          & 0.766          & 0.711          & 0.671          & 0.725 \\
U-Net               && 0.757          & 0.888          & 0.855          & 0.843          & 0.755          & 0.639          & 0.689          & 0.653          & 0.737 \\
DeepLabv3+          && 0.794          & 0.899          & 0.863          & 0.866          & 0.764          & \textbf{0.800} & 0.693          & 0.677          & 0.792 \\ 
DANet               && 0.775          & 0.900          & 0.853          & 0.852          & 0.772          & 0.713          & 0.682          & 0.715          & 0.712 \\ [3pt]

Inception-v3   && 0.716          & 0.895          & 0.893          & 0.865          & 0.766          & 0.500          & 0.540          & 0.594          & 0.678 \\ 
%ABN (BCE)           && 0.717          & \textbf{0.911} & 0.894          & 0.836          & 0.723          & 0.475          & 0.581          & 0.654          & 0.661 \\
%Inception-v3 (BCE)  && 0.719          & 0.900          & 0.897          & 0.858          & 0.759          & 0.475          & 0.556          & 0.623          & 0.682 \\
ABN-lesion && 0.726          & 0.900          & \textbf{0.900} & \textbf{0.871} & 0.761          & 0.519          & 0.552          & 0.627          & 0.678 \\ [3pt]

%\emph{Lesion-Net with Dice loss} \\
%Lesion-Net-8s            && 0.759          & 0.899          & 0.856          & 0.849          & 0.769          & 0.690          & 0.617          & 0.660          & 0.730 \\
%Lesion-Net-4s            && 0.765          & 0.900          & 0.862          & 0.849          & 0.763          & 0.674          & 0.645          & 0.655          & 0.771 \\
%Lesion-Net-2s            && 0.767          & 0.898          & 0.865          & 0.853          & 0.764          & 0.699          & 0.649          & 0.663          & 0.747 \\
%Lesion-Net-16s           && 0.769          & 0.899          & 0.860          & 0.851          & 0.754          & 0.709          & 0.661          & 0.694          & 0.724 \\

%\emph{Lesion-Net with Dual loss} \\
%Lesion-Net-32s  && 0.792          & 0.899          & 0.881          & 0.857          & 0.778          & 0.720          & \textbf{0.773} & 0.669          & 0.762 \\
Lesion-Net          && \textbf{0.801} & 0.902          & 0.882          & 0.866          & 0.792          & 0.733          & 0.726          & 0.701          & \textbf{0.807} \\
%Lesion-Net-8s            && 0.780          & 0.900          & 0.881          & 0.861          & 0.771          & 0.687          & 0.693          & 0.711          & 0.733 \\
%Lesion-Net-4s            && 0.781          & 0.904          & 0.883          & 0.862          & 0.791          & 0.678          & 0.660          & \textbf{0.719} & 0.748 \\
%Lesion-Net-2s            && 0.787          & 0.900          & 0.893          & 0.868          & \textbf{0.793} & 0.706          & 0.706          & 0.667          & 0.764 \\


\bottomrule
\end{tabular}}
\end{table}


==> table-loss.tex <==


\begin{table} [tb!]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{Performance of Lesion-Net-16s with different losses}. }
\label{tab:loss}
\scalebox{0.9}{
\begin{tabular}{@{}ll r r@{}}
\toprule
\textbf{Loss}      && \textbf{Lesion segmentation} &\textbf{Lesion classification}    \\
\cmidrule{1-1}  \cmidrule{2-4}
\emph{Lesion-Net-16s}: \\
Weighted cross-entropy  && 0.365  & 0.533 \\
Focal loss              && 0.504  & 0.635 \\
Dice                && \textbf{0.594}  & 0.769 \\
\emph{Dual loss (this paper)}               && 0.591  & \textbf{0.801} \\ [3pt]

\bottomrule
\end{tabular}}
\end{table}
